Biased or Flawed? Mitigating Stereotypes in Generative Language Models by Addressing Task-Specific Flaws

Recent studies have shown that generative language models often reflect and amplify societal biases in their outputs. However, these studies frequently conflate observed biases with other task-specific shortcomings, such as comprehension failure. For example, when a model misinterprets a text and produces a response that reinforces a stereotype, it becomes difficult to determine whether the issue arises from inherent bias or from a misunderstanding of the given content. In this paper, we conduct a multi-faceted evaluation that distinctly disentangles bias from flaws within the reading comprehension task. We propose a targeted stereotype mitigation framework that implicitly mitigates observed stereotypes in generative models through instruction-tuning on general-purpose datasets. We reduce stereotypical outputs by over 60% across multiple dimensions -- including nationality, age, gender, disability, and physical appearance -- by addressing comprehension-based failures, and without relying on explicit debiasing techniques. We evaluate several state-of-the-art generative models to demonstrate the effectiveness of our approach while maintaining the overall utility. Our findings highlight the need to critically disentangle the concept of `bias' from other types of errors to build more targeted and effective mitigation strategies. CONTENT WARNING: Some examples contain offensive stereotypes.

==> sections/tables/instr_unfair.tex <==
\begin{table}[t]
\centering
\small
\begin{tabular}{lrrr}
\toprule
\textbf{Model} & \textbf{Overall} & \textbf{Amb} & \textbf{Disamb} \\
\midrule
Llama2-7B   & 71.03 & 82.84 & 69.22 \\
Llama2-13B  & 73.36 & 87.69 & 68.80 \\
Mistral   & -- & -- & -- \\
Mixtral     & -- & -- & -- \\
Phi-2       & 64.50 & 74.60 & 64.23 \\
\bottomrule
\end{tabular}
\caption{EMO scores measuring regional stereotypes
using the BBQ dataset \textit{after instruction-tuning}. Lower values indicate worse performance.}
\label{tab:instr_unfair}
\end{table}


==> sections/tables/stats.tex <==
\begin{table}[t]
    \centering
    \small
    \begin{tabular}{lp{1cm}p{1cm}p{1.2cm}}
        \toprule
        \textbf{Dataset} & \textbf{\#Overall} & \textbf{\#Ambig} & \textbf{\#Disambig} \\
        \midrule
        BBQ (Nationality) & 3,080 & 1,540 & 1,540 \\
        SQuAD-v2 (Overall) & 11,873 & 5,945 & 5,926 \\
        SQuAD-v2 (Identity) & 3,357 & 1,663 & 1,694 \\
        SQuAD-v2 (Non-Id) & 8,514 & 4,282 & 4,232 \\
        Instruction-Tuning & 284,592 & 142,296 & 142,296 \\
        \bottomrule
    \end{tabular}
    \caption{Dataset stats for overall, ambiguous, and disambiguous contexts for instruction-tuning and evaluation.}
    \label{tab:data_stats1}
\end{table}

